Time-to-Event Pretraining for 3D Medical Imaging

With the rise of medical foundation models and the growing availability of imaging data, scalable pretraining techniques offer a promising way to identify imaging biomarkers predictive of future disease risk. While current self-supervised methods for 3D medical imaging models capture local structural features like organ morphology, they fail to link pixel biomarkers with long-term health outcomes due to a missing context problem. Current approaches lack the temporal context necessary to identify biomarkers correlated with disease progression, as they rely on supervision derived only from images and concurrent text descriptions. To address this, we introduce time-to-event pretraining, a pretraining framework for 3D medical imaging models that leverages large-scale temporal supervision from paired, longitudinal electronic health records (EHRs). Using a dataset of 18,945 CT scans (4.2 million 2D images) and time-to-event distributions across thousands of EHR-derived tasks, our method improves outcome prediction, achieving an average AUROC increase of 23.7% and a 29.4% gain in Harrell's C-index across 8 benchmark tasks. Importantly, these gains are achieved without sacrificing diagnostic classification performance. This study lays the foundation for integrating longitudinal EHR and 3D imaging data to advance clinical risk prediction.

==> 3_methods.tex <==
\begin{figure*}[ht]
\begin{center}
\includegraphics[width=0.95\textwidth]{Figures/Figure_1_V7.pdf}
\end{center}
   \caption{Overview of the proposed \textit{future-guided pretraining} pipeline. We conduct continued pretraining of an existing vision model by incorporating future medical events from patients' EHR timelines as time-to-event (TTE) supervision. The resulting encoder is then frozen and adapted via a non-linear task head.} 
\label{fig:method}
%\vspace{0.1in}
\end{figure*}




\section{Future-guided pretraining for Image models}
\label{Methodology}
For survival modeling, the goal is to estimate the distribution of survival times $T$, also known as the time until an event of interest. One complexity is that medical data is often right censored, where the survival time $T$ is not always observed due to a limited followup period. With right-censoring, we don't observe $T$ and instead observe time $\tilde{T} = \min (T, C)$, where the $C$ is the censoring time. The observable data is denoted as $\mathcal{O} = \bigl\{ (\tilde{T}_i, \Delta_i, X_i^T): i=1, ..., n\bigr\}$, where $X_i$ is the features of observation $i$ and $\Delta=I(T\leq C)$ is an event indicator function whose value is $1$ when the actual event time is observed.  When $\Delta=0$, we do not know the true survival time, but we know that it is greater than $\tilde{T}_i$. The mixture of known survival times and censored survival times necessitates the use of special survival modeling methods that can estimate $T$ in an unbiased manner despite the censorship. For all of our survival models (both pretraining and fine-tuning), we use the piecewise exponential neural network (PEANN) approach \cite{peann}, where a neural network is used to approximate the parameters of a piecewise exponential distribution. For pretraining in particular, we also need a selection of survival tasks to use as a pretraining set. Following prior work \cite{steinberg2023motor}, we construct a pretraining task set by ranking medical codes by Shannon entropy \cite{shannon1948mathematical} and then picking the top 8,192 codes. This set represents the most informative codes to cover a broad spectrum of clinical events. Thus the continued pretraining step can be deemed as a massive multitask learning with a survival objective, as show Figure \ref{fig:method} (B).

\textbf{Defining the piecewise exponential distribution}: \\
Piecewise neural networks (PEANN) provide a simple and flexible approach for survival modeling by having a neural network provide the parameters of a piecewise exponential distribution \cite{peann}. We use PEANN for this work because it has a variety of advantages, the most important of which is that unlike other methods such as DeepSurv (aka Cox) PEANN does not require every batch to have uncensored examples. This is important for pretraining since many of our tasks are highly censored, and large images mean that batch sizes are very small.

In order to implement PEANN, we have to define the survival function as a piecewise exponential distribution. We select the number of pieces, $P$, and divide the response period into $P$ pieces, where each piece covers the response period starting at $S_p$ and ending at $E_p$. For every piece $p$ and image $i$ in our dataset, our model needs to output $\lambda_{ip}$, the instantaneous hazard rate for the patient described by that image during the response time period $p$. These $\lambda$ values are then used to define a survival function for each image $i$:

\begin{equation}
    S_{i}(t) = \prod_{p=1}^P \exp\bigl[-\lambda_{ip}*(\min (t, E_p)-S_p))*I(t\geq S_p)\bigr],
\end{equation}

The PDF of the survival distribution, $f$, is then simply the negative of the derivative of the survival function.

\begin{equation}
    f_{i} = -\frac{\partial S_{i}}{\partial t}
\end{equation}

We define the loss function for training by using the survival function to implement the standard survival likelihood equation and taking the product of that likelihood over the entire dataset. 

\begin{equation}
\begin{aligned}
    \mathcal{L} &= \prod_{i=i}^n [S_{i}(t)]^{1-\delta_{i}}\left[f_{i}(t)\right]^{\delta_{i}} \\
\end{aligned}
\end{equation}



\textbf{Connecting the image model to the piecewise exponential distribution}: \\
In order to train our image models using PEANN, we have to parameterize $\lambda{ip}$ (the instantaneous hazard rates that define our piecewise exponential distribution) as a function of our image neural network. We start with an image backbone neural network $h$, that takes as input an image $X_i$ and outputs an intermediate representation $Z_i$. 

\begin{equation}
\begin{aligned}
    & h: \mathbb{R}^n \rightarrow \mathbb{R}^m \\
    & Z_{i} = h(X_i),
\end{aligned} 
\end{equation}

We need a vector of length $P$ for every image, so we apply a linear layer to resize $Z_i$. $M_{i} = linear(Z_{i})$. Finally, we apply an exponential transformation to obtain a $\lambda$ vector of length $P$ for every image. $\lambda_{i} = exp(M_{i})$.



% \subsection{Continued pretraining with TTE loss}
% Traditionally survival function is defined as:
% $
%     S(t) := Pr(T > t) = e^{-\int_0^t \lambda(t)dt}.
% $
% It measures the probability of a patient surviving up until the time $t$ (not experience the event), where $T$ is a continuous random variable with probability density function (PDF) as $f(t)=\lambda e^{-\lambda t}$, and therefore cumulative density function (CDF) is $F(t)=Pr(T<t)=1-S(t)$. The instantaneous hazard is:
% \begin{equation}
%     \lambda(t) := \lim_{dt\rightarrow0}\frac{Pr(t<T<t+dt|T>t)}{dt}
% \end{equation}
% Different time-to-event models use different definitions to model the instantaneous hazard $\lambda(t)$. We here use a piecewise exponential function \cite{kitchin1983new} where $\lambda(t)$ has a constant baseline hazard and is only dependent on the patient's attribute in a timepiece $p(t)$. This is different from Cox proportional hazard where the baseline hazard is constant in each time piece. To have multiple timepieces $p(t)$ and multiple events of interest $j$, each timepiece has $\lambda_{ijp(t)}=C_{ijp}$ where $C$ is a function that is dependent on the patient $i$ but not on time for event $j$.

% To make use of deep learning models, we use a neural network to define $C_{ijp}$. We first need to use the neural network to derive patient representation $M_{ijp}$ for patient $i$'s information at timepiece $p$ for event $j$. Since we will use exponential function for survival data, we therefore have
% \begin{equation}
%     \lambda_{ijp} = C_{ijp} = \exp (A*M_{ijp}+b),
%     \label{exponential_function}
% \end{equation}
% where $A$ and $b$ are learned parameters for the survival function. With the hazard calculated, we can then input it into the survival function:
% \begin{equation}
%     S_{ij}(t) = \prod_{p=1}^P \exp\bigl[-\lambda_{ijp}*\min (t, E_p)-S_p)*I(t\geq S_p)\bigr],
% \end{equation}
% where each timepiece $p$ has a starting point $S_p$ and end point $E_p$ and $I(\cdot)$ is an indicator function. The likelihood of the observed data for patient $i$ and event $j$ is:
% \begin{equation}
% \begin{aligned}
%     \mathcal{L}_{ij} &= \prod_{p=1}^P [S_{ijp}(t)]^{1-\delta_{ijp}}[f_{ijp}(t)]^{\delta_{ijp}} \\
% \end{aligned}
% \end{equation}
% where $\delta_{ijp}$ is event indicator whose value is 1 when patient $i$ has event $j$ at timepiece $p$. The probability density function has the form $\lambda_{ijp}S_{ijp}(t)$.



% We therefore can construct the negative log likelihood (NLL) as loss function for the model:
% \begin{equation}
% \begin{aligned}
%     -\log\mathcal{L}_{ij} &= -\sum_{p=1}^P (1-\delta_{ijp})\log S_{ijp}(t) + \delta_{ijp}\log(\lambda_{ijp}S_{ijp}(t)) \\
%     &= -\sum_{p=1}^P \log S_{ijp}(t) + \delta_{ijp}\log\lambda_{ijp}
% \end{aligned}    
% \end{equation}




% \subsection{Image model training}
% To illustrate the generalizability of continued TTE pretraining, we conducted the experiments on different model architectures. We poised our method as continued pretraining method so the image backbone is already pretrained with various techniques and can be agnostic to the continued pretraining, therefore we can simply deem it as a feature extractor for downstream TTE loss calculation:
% \begin{equation}
% \begin{aligned}
%     & h: \mathbb{R}^n \rightarrow \mathbb{R}^m \\
%     & Z_{i} = h(X_i),
% \end{aligned} 
% \end{equation}
% where $X_i$ is patient $i$'s input image and after feature extractor $h$ we can derive the intermediate feature $Z_i$ which can carry the information from pretrained pipeline (e.g. readily useful for segmentation if pretrained on patch reconstruction pipeline). Next, the feature will be fed into survival head and each head will produce the embedding of a specific event $j$ with respect to patient $i$:
% \begin{equation}
% \begin{aligned}
%     & f_j: \mathbb{R}^m \rightarrow \mathbb{R}^l \\
%     & M_{ijp} = f_j(Z_i), \text{where} \ p=1, ..., P.
% \end{aligned} 
% \end{equation}
% The task head will derive the features for patient $i$ on event $j$ at timepiece $p$. The feature $M_{ijp}$ will be used to calculate the TTE loss per Eq. (\ref{exponential_function}). 




\begin{table}[t]
\centering
\small
\begin{tabular}{lccccccc}
\toprule
\textbf{Name} & \textbf{Dim.} & \textbf{Region} & \textbf{Train/Test} & \textbf{Tasks}  \\
\midrule
INSPECT \cite{huang2024inspect}   & 3D & Chest CT     & 18,945/3,214  & 4  \\
RSPECT  \cite{colak2021rsna}   & 3D & Chest CT     & 12,195/2,810 & 13  \\
% CheXpert*  & 2D & Chest X-Ray  & 496   & 14 \\
\bottomrule
\end{tabular}
\caption{Dataset statistics. Note for INSPECT, both diagnosis and prognosis labels are present, and RSPECT only has diagnosis labels.}
\label{dataset}
\end{table}





==> 7_a_contribution_table.tex <==
\begin{table}[h]
    \centering
    \resizebox{1.05\textwidth}{!}{
    \begin{tabular}{lccccccc}
        \toprule
        & Conceptualization & Funding acquisition & Investigation & Methodology & Resources & Code implementation & Writing \\
        \midrule
        Zepeng Huo*   & x & x & x & x & & x & x \\
        Jason Alan Fries*     & x & & x & x & & & x \\
        Alejandro Lozano* & x & & x & & & x & x \\
        Jeya Maria Jose Valanarasu       & x & & & & & & \\
        Ethan Steinberg      & & & x & x & & x & x \\
        Louis Blankemeier   & & & x & x & & x & x \\
        Akshay S. Chaudhar  & & & x & x & & x & x \\
        Curtis Langlotz  & & x &  & x & & x & x \\
        Nigam H. Shah      & & x & x & & x & x & x \\
        \bottomrule
    \end{tabular}}
    \caption{Author Contributions}
    \label{tab:author_contributions}
\end{table}


==> tables/OLD/copy_wrong.tex <==




\begin{table}[h]
    \centering
    \caption{Pulmonary embolism diagnosis  breakdown by subgroups. Boostraped (n=1000)  AUROC  ($\uparrow$)  of base model compared to TTE continue pretrained model across subgroups categories. Bold indicates the best performance across all models. }
    \begin{tabular}{@{}llccc@{}}
        \toprule
        Group     & Concept                       & \SwinUNETR\ \base\         & \SwinUNETR\ \SV\           & \SwinUNETR\ \TTE\          \\ \midrule
        Gender    & Female                        & 0.548 (0.484, 0.614) & 0.554 (0.519, 0.590)* & \textbf{0.589 (0.558, 0.620)}* \\
                  & Male                          & \textbf{0.658 (0.581, 0.738)} & 0.583 (0.545, 0.621)* & 0.573 (0.534, 0.611)* \\ \midrule
        Age       & 18-39                        & \textbf{0.632 (0.509, 0.754)} & 0.598 (0.523, 0.673)* & 0.600 (0.535, 0.664)* \\
                  & 39-69                        & 0.566 (0.487, 0.641) & 0.573 (0.536, 0.611)* & \textbf{0.603 (0.570, 0.636)}* \\
                  & 69-89                        & \textbf{0.630 (0.545, 0.714)} & 0.547 (0.502, 0.590)* & 0.552 (0.506, 0.598)* \\
                  & $>$89                          & 0.470 (0.203, 0.722) & \textbf{0.538 (0.417, 0.655)}* & 0.524 (0.381, 0.665)* \\ \midrule
        Race      & Asian                         & \textbf{0.626 (0.499, 0.759)} & 0.536 (0.472, 0.600)* & 0.617 (0.552, 0.686)* \\
                  & Black                         & \textbf{0.683 (0.503, 0.853)} & 0.652 (0.556, 0.743)*& 0.668 (0.597, 0.744)* \\
                  & Native                        & 0.261 (0.000, 0.800) & 0.265 (0.141, 0.414)& \textbf{0.563 (0.354, 0.768)}* \\
                  & Unknown                       & \textbf{0.670 (0.562, 0.781)} & 0.589 (0.531, 0.647)* & 0.599 (0.544, 0.652)* \\
                  & White                         & 0.560 (0.492, 0.627) & \textbf{0.568 (0.536, 0.601)}* & 0.556 (0.523, 0.590)* \\ \midrule
        Ethnicity  & Hispanic or Latino           & \textbf{0.661 (0.535, 0.779)} & 0.596 (0.529, 0.656)* & 0.563 (0.501, 0.624)* \\
                  & Not Hispanic or Latino       & 0.581 (0.524, 0.637) & 0.563 (0.533, 0.591)* & \textbf{0.588 (0.559, 0.616)}\\
                  & Unknown                       & 0.479 (0.143, 0.817) & 0.561 (0.456, 0.675)* & \textbf{0.597 (0.489, 0.714)}* \\ 
        \bottomrule
    \end{tabular}
    \label{tab:pe_positive_nlp}
\end{table}


\begin{table}[ht]
    \centering
    \caption{1-Month Mortality}
    \begin{tabular}{@{}llccc@{}}
        \toprule
        Group & Concept & \SwinUNETR\ \base\ & \SwinUNETR\ \SV\ & \SwinUNETR\ \TTE\ \\
        \midrule
        Gender & Female & 0.686 (0.610, 0.761) & 0.687 (0.638, 0.732) & \textbf{0.781 (0.743, 0.820)}*\\
        & Male & 0.627 (0.498, 0.757) & 0.709 (0.658, 0.766)* & \textbf{0.799 (0.760, 0.837)}*\\
        \midrule
        Age & 18-39 & 0.724 (0.598, 0.824) & 0.722 (0.594, 0.847) & \textbf{0.791 (0.688, 0.879)}*\\
        & 39-69 & 0.612 (0.501, 0.723) & 0.688 (0.634, 0.737)* & \textbf{0.807 (0.769, 0.841)}* \\
        & 69-89 & 0.654 (0.525, 0.770) & 0.693 (0.628, 0.756)* & \textbf{0.767 (0.716, 0.815)}* \\
        & $>$89 & \textbf{0.827 (0.529, 1.000)} & 0.681 (0.485, 0.858)* & 0.637 (0.463, 0.813)* \\
        \midrule
        Race & Asian & 0.673 (0.545, 0.797) & 0.701 (0.608, 0.787)* & \textbf{0.796 (0.732, 0.860)}*  \\
        & Black & 0.743 (0.389, 0.989) & 0.718 (0.588, 0.837)* & \textbf{0.808 (0.713, 0.895)}* \\
        & Native & 0.608 (0.091, 1.000) & 0.618 (0.340, 0.98)& \textbf{0.709 (0.380, 0.920)}* \\
        & Unknown & 0.703 (0.558, 0.836) & 0.727 (0.655, 0.789)* & \textbf{0.765 (0.703, 0.824)}* \\
        & White & 0.633 (0.538, 0.731) & 0.681 (0.633, 0.732)* & \textbf{0.797 (0.761, 0.833)}*  \\
        \midrule
        Ethnicity & Hispanic or Latino & 0.577 (0.356, 0.791)* & 0.680 (0.596, 0.762) & \textbf{0.768 (0.686, 0.842)} * \\
        & Not Hispanic or Latino & 0.671 (0.598, 0.744) & 0.697 (0.656, 0.737)* & \textbf{0.793 (0.762, 0.822)}*  \\
        & Unknown & 0.710 (0.550, 0.850) & 0.752 (0.531, 0.934)* & \textbf{0.776 (0.634, 0.894)}*  \\
        \bottomrule
    \end{tabular}
\end{table}


\begin{table}[ht]
    \centering
    \caption{6-Month Mortality AUROC The 95 \% confidence interval for the difference is also included.}
    \begin{tabular}{@{}llccc@{}}
        \toprule
        Group & Concept & \SwinUNETR\ \base\ & \SwinUNETR\ \SV\ & \SwinUNETR\ \TTE\ \\ \midrule
        \multirow{2}{*}{Gender} & Female & 0.585 (0.502, 0.666) & 0.656 (0.619, 0.692)* & \textbf{0.769 (0.739, 0.798)}*\\
                                & Male   & 0.561 (0.450, 0.666) & 0.708 (0.661, 0.753)* & 
                                \textbf{0.793 (0.758, 0.827)}* \\  \midrule
        \multirow{4}{*}{Age}    & 18-39  & 0.506 (0.280, 0.738) & 0.644 (0.550, 0.731)* & \textbf{0.849 (0.788, 0.906)}*\\ 
                                & 39-69  & 0.570 (0.473, 0.659) & 0.710 (0.672, 0.746)* &\textbf{ 0.778 (0.749, 0.807)}*\\
                                & 69-89  & 0.581 (0.479, 0.686) & 0.629 (0.577, 0.681)* & \textbf{0.752 (0.709, 0.794)}*\\
                                & $>$ 89    & 0.548 (0.200, 1.000) & 0.558 (0.399, 0.721) & \textbf{0.729 (0.559, 0.884)}*\\  \midrule
        \multirow{5}{*}{Race}   & Asian   & 0.540 (0.360, 0.709) & 0.677 (0.601, 0.757)* & \textbf{0.737 (0.661, 0.808)}* \\
                                & Black   & 0.700 (0.475, 0.925) & 0.638 (0.524, 0.752)* & \textbf{0.852 (0.780, 0.920)}* \\
                                & Native  & 0.888 (0.630, 1.000) & 0.652 (0.375, 0.912)* & \textbf{0.916 (0.774, 1.000)}*\\
                                & Unknown  & 0.655 (0.484, 0.819) & 0.660 (0.595, 0.724) & \textbf{0.737 (0.689, 0.787)}*\\
                                & White   & 0.515 (0.427, 0.600) & 0.688 (0.651, 0.723)* & \textbf{0.789 (0.763, 0.815)}*\\ \midrule
        \multirow{3}{*}{Ethnicity} & Hispanic or Latino & 0.666 (0.496, 0.825) & 0.668 (0.592, 0.739) & \textbf{0.725 (0.658, 0.790)}* \\
                                  & Not Hispanic or Latino & 0.559 (0.489, 0.632) & 0.676 (0.643, 0.709)* & \textbf{0.787 (0.763, 0.811)}*\\
                                  & Unknown & 0.592 (0.333, 0.827) & 0.732 (0.589, 0.862)* &\textbf{ 0.808 (0.725, 0.883)}* \\ 
        \bottomrule
    \end{tabular}
\end{table}


\begin{table}[ht]
    \centering
    \caption{12-Month Mortality}
    \begin{tabular}{@{}lll l l@{}}
        \toprule
        \textbf{Group} & \textbf{Concept} & \SwinUNETR\ \base\ & \SwinUNETR\ \SV\ & \SwinUNETR\ \TTE\ \\
        \midrule
        Gender& Female & 0.560 (0.495, 0.625) & 0.669 (0.637, 0.702)* & \textbf{0.760 (0.734, 0.786)}* \\
                       & Male   & 0.594 (0.496, 0.689) & 0.700 (0.661, 0.738)* & \textbf{0.770 (0.737, 0.802)}* \\
        \midrule
        Age   & 18-39  & 0.689 (0.546, 0.828) & 0.654 (0.569, 0.738)* & \textbf{0.852 (0.787, 0.908)}* \\
                       & 39-69  & 0.575 (0.502, 0.645) & 0.713 (0.681, 0.745)* & \textbf{0.774 (0.745, 0.801)}*\\
                       & 69-89  & 0.565 (0.46, 0.666) & 0.628 (0.582, 0.672)* & \textbf{0.727 (0.689, 0.764)}* \\
*                       & $>$89    & 0.355 (0.056, 0.68) & 0.601 (0.450, 0.750)* & \textbf{0.614 (0.467, 0.766)}* \\
        \midrule
        Race  & Asian   & 0.519 (0.397, 0.635) & 0.687 (0.619, 0.751)* & \textbf{0.712 (0.652, 0.767)}* \\
                       & Black   & 0.678 (0.462, 0.881) & 0.667 (0.566, 0.76)* & \textbf{0.782 (0.694, 0.859)}*\\
                       & Native  & \textbf{0.935 (0.771, 1.0)} & 0.705 (0.525, 0.885)* & 0.819 (0.667, 0.95)* \\
                       & Unknown  & 0.594 (0.441, 0.738) & 0.649 (0.589, 0.706)* & \textbf{0.746 (0.700, 0.794)}* \\
                       & White   & 0.538 (0.474, 0.605) & 0.694 (0.661, 0.726)* & \textbf{0.782 (0.756, 0.808)}* \\
        \midrule
        Ethnicity & Hispanic or Latino & 0.613 (0.467, 0.753) & 0.629 (0.555, 0.704)* & \textbf{0.718 (0.659, 0.779)}* \\
                       & Not Hispanic or Latino & 0.583 (0.527, 0.646) & 0.689 (0.66, 0.717)* & \textbf{0.771 (0.748, 0.793)}*\\
                       & Unknown  & 0.264 (0.067, 0.467) & 0.732 (0.595, 0.855)* & \textbf{0.799 (0.713, 0.876)}* \\
        \bottomrule
    \end{tabular}
\end{table}




\begin{table}[ht]
    \centering
    \caption{1-Month Readmission}
    \begin{tabular}{@{}llccc@{}}
        \toprule
        Group         & Concept                  & \SwinUNETR\ \base\          & \SwinUNETR\ \SV\             & \SwinUNETR\ \TTE\       \\ \midrule
        Gender        & Female                   & \textbf{0.629 (0.505, 0.763)} & 0.593 (0.529, 0.657)* & 0.609 (0.542, 0.676)* \\
                      & Male                     & \textbf{0.654 (0.550, 0.759)}  & 0.512 (0.436, 0.588)* & 0.625 (0.535, 0.709)* \\ \midrule
        Age           & 18-39                   & \textbf{0.619 (0.417, 0.826)} & 0.403 (0.274, 0.543)* & 0.560 (0.438, 0.679)* \\
                      & 39-69                   & \textbf{0.604 (0.487, 0.721)} & 0.602 (0.535, 0.668) & 0.595 (0.528, 0.661)* \\
                      & 69-89                   & \textbf{0.719 (0.559, 0.874)} & 0.571 (0.480, 0.658)* & 0.694 (0.589, 0.794)* \\
                      & $>$89                     &               0.676 (0.461, 0.880)        & 0.648 (0.452, 0.838)* & \textbf{0.698 (0.467, 0.933)}*\\ \midrule
        Race          & Asian                    & 0.515 (0.179, 0.849) & 0.529 (0.419, 0.640) & \textbf{0.528 (0.380, 0.661)}\\
                      & Black                    & 0.530 (0.311, 0.745) & 0.554 (0.284, 0.801)* & \textbf{0.729 (0.491, 0.935)}* \\
                      & Native                   &  0.564 (0.461, 0.665)  & 0.678 (0.571, 0.780)* & \textbf{0.802 (0.708, 0.898)}* \\
                      & Unknown                  & \textbf{0.623 (0.425, 0.816)} & 0.588 (0.482, 0.690)* & 0.581 (0.458, 0.696)* \\
                      & White                    & \textbf{0.671 (0.581, 0.761)}& 0.559 (0.488, 0.625)* & 0.637 (0.572, 0.701)* \\ \midrule
        Ethnicity     & Hispanic or Latino       & 0.606 (0.326, 0.885) & \textbf{0.663 (0.531, 0.790)}* & 0.622 (0.450, 0.786)* \\
                      & Not Hispanic or Latino   & \textbf{0.648 (0.564, 0.733)} & 0.556 (0.502, 0.611)* & 0.633 (0.575, 0.686)* \\
                      & Unknown                  & \textbf{0.567 (0.059, 0.944)} & 0.455 (0.255, 0.674* & 0.419 (0.196, 0.667)* \\ \bottomrule
                      & Unknown                  & \textbf{0.567 (0.059, 0.944)} & 0.455 (0.255, 0.674)* & 0.419 (0.196, 0.667)* \\ \bottomrule
    \end{tabular}
\end{table}

\begin{table}[h]
    \centering
    \caption{6-Month Readmission}
    \begin{tabular}{@{}llccc@{}}
        \toprule
        Group & Concept & \SwinUNETR\ \base\ & \SwinUNETR\ \SV\ & \SwinUNETR\ \TTE\ \\ 
        \midrule
        \multirow{2}{*}{Gender} & Female & 0.536 (0.450, 0.620) & 0.558 (0.515, 0.600)* & \textbf{0.631 (0.592, 0.671)}*\\ 
        & Male & 0.554 (0.462, 0.649) & 0.537 (0.483, 0.592)*  & \textbf{0.615 (0.567, 0.661)}*\\ 
        \midrule
        \multirow{4}{*}{Age} & 18-39 & 0.449 (0.322, 0.582) & 0.500 (0.422, 0.574)*  & \textbf{0.632 (0.547, 0.712)}*\\ 
        & 39-69 & 0.540 (0.457, 0.620) & 0.550 (0.506, 0.592)*  & \textbf{0.617 (0.575, 0.660)}*\\ 
        & 69-89 & 0.635 (0.500, 0.769) & 0.586 (0.524, 0.648)*  & \textbf{0.642 (0.578, 0.708)}* \\ 
        & $>$89 & 0.621 (0.385, 0.846) & 0.483 (0.190, 0.766)*  & \textbf{0.737 (0.406, 0.952)}* \\ 
        \midrule
        \multirow{5}{*}{Race} & Asian & 0.589 (0.421, 0.757) & 0.496 (0.416, 0.574)*  & \textbf{0.597 (0.516, 0.674)}* \\ 
        & Black & \textbf{0.739 (0.561, 0.908)}& 0.568 (0.403, 0.724)*  & 0.629 (0.488, 0.762)* \\ 
        & Native & \textbf{0.724 (0.455, 0.909)}& 0.623 (0.346, 0.867)*  & 0.667 (0.405, 0.937)* \\ 
        & Unknown & 0.516 (0.361, 0.676) & 0.568 (0.503, 0.631)*  & \textbf{0.569 (0.502, 0.635)}*\\ 
        & White & 0.518 (0.439, 0.598) & 0.555 (0.511, 0.598)*  & \textbf{0.654 (0.616, 0.692)}*\\ 
        \midrule
        \multirow{3}{*}{Ethnicity} & Hispanic or Latino & 0.504 (0.273, 0.757)*  & \textbf{0.618 (0.520, 0.705)}*  & 0.597 (0.498, 0.688)* \\ 
        & Not Hispanic or Latino & 0.547 (0.482, 0.610) & 0.545 (0.508, 0.581)  & \textbf{0.633 (0.601, 0.664)}* \\ 
        & Unknown & 0.401 (0.062, 0.711) & 0.473 (0.352, 0.584)*  &\textbf{ 0.573 (0.412, 0.727)}*\\ 
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[h]
    \centering
    \caption{12 Month Readmission}
    \begin{tabular}{@{}llccc@{}}
        \toprule
        Group & Concept & \SwinUNETR\ \base\ & \SwinUNETR\ \SV\ & \SwinUNETR\ \TTE\ \\ \midrule
        Gender & Female & 0.519 (0.451, 0.587) & 0.540 (0.504, 0.579)*  & \textbf{0.617 (0.578, 0.654)}*\\
               & Male   & 0.514 (0.433, 0.603) & 0.487 (0.445, 0.531)*  & \textbf{0.579 (0.537, 0.622)}* \\ \midrule
        Age    & 18-39  & 0.600 (0.473, 0.731) & 0.513 (0.442, 0.578)*  & \textbf{0.669 (0.599, 0.734)}* \\
               & 39-69  & 0.472 (0.407, 0.543) & 0.502 (0.462, 0.542)*  & \textbf{0.576 (0.539, 0.615)}* \\
               & 69-89  & 0.551 (0.408, 0.694) & 0.538 (0.482, 0.596)*  & \textbf{0.611 (0.556, 0.668)}* \\
               & $>$89    & \textbf{0.752 (0.545, 0.917)}& 0.680 (0.307, 0.963)*  & 0.693 (0.421, 0.904)* \\ \midrule
        Race   & Asian  & 0.468 (0.316, 0.620) & 0.572 (0.495, 0.648)*  & \textbf{0.576 (0.512, 0.646)}* \\
               & Black  & 0.577 (0.346, 0.798) & 0.412 (0.263, 0.564)*  & \textbf{0.592 (0.454, 0.728)}* \\
               & Native & 0.722 (0.500, 0.909) & 0.743 (0.551, 0.921)*  & \textbf{0.863 (0.647, 1.000)}* \\
               & Unknown & 0.436 (0.312, 0.557) & 0.514 (0.460, 0.567)*  & \textbf{0.525 (0.465, 0.583)}*\\
               & White   & 0.536 (0.467, 0.606) & 0.502 (0.461, 0.541)*  & \textbf{0.628 (0.591, 0.665)}* \\ \midrule
        Ethnicity & Hispanic or Latino & 0.442 (0.318, 0.570) & 0.510 (0.441, 0.579)*  & \textbf{0.565 (0.494, 0.635)}* \\
                  & Not Hispanic or Latino & 0.532 (0.471, 0.593) & 0.520 (0.488, 0.553)*  & \textbf{0.612 (0.581, 0.644)}* \\
                  & Unknown & \textbf{0.554 (0.192, 1.000)} & 0.478 (0.353, 0.610)*  & 0.526 (0.387, 0.673)* \\ 
        \bottomrule
    \end{tabular}
\end{table}


\begin{table}[ht]
    \centering
    \caption{12 Month PH}
    \begin{tabular}{@{}llccc@{}}
        \toprule
        Group & Concept & \SwinUNETR\ \base\ & \SwinUNETR\ \SV\ & \SwinUNETR\ \TTE\ \\ \midrule
        \multirow{2}{*}{Gender} & Female & 0.503 (0.424, 0.585) & 0.561 (0.521, 0.603)*  & \textbf{0.601 (0.559, 0.643)*}\\
                                & Male   & 0.507 (0.389, 0.625) & 0.567 (0.522, 0.615)*  & \textbf{0.615 (0.572, 0.658)}* \\ \midrule
        \multirow{4}{*}{Age}    & 18-39  & 0.577 (0.452, 0.725) & 0.595 (0.474, 0.711)*  & \textbf{0.750 (0.659, 0.831)}*\\
                                & 39-69  & 0.422 (0.334, 0.517) & 0.558 (0.514, 0.603)*  & \textbf{0.602 (0.560, 0.644)}* \\
                                & 69-89  & \textbf{0.584 (0.475, 0.686)} & 0.537 (0.481, 0.591)*  & 0.569 (0.515, 0.622) \\
                                & $>$89    & 0.530 (0.100, 0.958) & \textbf{0.548 (0.404, 0.698)}*  & 0.454 (0.312, 0.602)* \\ \midrule
        \multirow{5}{*}{Race}   & Asian   & 0.519 (0.297, 0.728) & 0.490 (0.410, 0.575)*  & \textbf{0.583 (0.504, 0.663)}*\\
                                & Black   & 0.558 (0.277, 0.811) & \textbf{0.677 (0.525, 0.816)}*  & 0.615 (0.490, 0.732)* \\
                                & Native  & \textbf{0.554 (0.200, 0.900)} & 0.373 (0.162, 0.613)*  & 0.465 (0.231, 0.695)*\\
                                & Unknown  & 0.398 (0.276, 0.527) & \textbf{0.586 (0.520, 0.649)}* & 0.536 (0.467, 0.605)* \\
                                & White   & 0.559 (0.466, 0.650) & 0.574 (0.531, 0.615)*  & \textbf{0.648 (0.606, 0.689)}* \\ \midrule
        \multirow{3}{*}{Ethnicity} & Hispanic or Latino  & 0.343 (0.236, 0.459) & \textbf{0.605 (0.529, 0.678)}* & 0.548 (0.471, 0.626)* \\
                                & Not Hispanic or Latino & 0.556 (0.476, 0.642) & 0.553 (0.517, 0.586)*  & \textbf{0.623 (0.587, 0.656)} \\
                                & Unknown & 0.531 (0.438, 0.617)  & \textbf{0.591 (0.422, 0.746)}*  & 0.478 (0.317, 0.640)*  \\ \bottomrule
    \end{tabular}
\end{table}




==> tables/OLD/integrated_brier_score.tex <==
\begin{table*}[h!]
\centering
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{l c c c c c c c c}
\toprule
\multirow{2}{*}{\textbf{Model}}  & \multicolumn{8}{c}{\textbf{Integrated Brier Score} \downarrow} \\ \cmidrule(lr){2-9}
& \textbf{Mortality} & \textbf{Readmission} & \textbf{Pulmonary Hypertension} & \textbf{Atelectasis} & \textbf{Cardiomegaly} & \textbf{Consolidation} & \textbf{Edema} & \textbf{Pleural Effusion} \\
\midrule
\SwinUNETR\ \base\ & 0.075 & 0.071 & 0.072 & 0.094 & 0.087 & 0.104 & 0.099 & 0.091 \\
\SwinUNETR\ \MT\  & 0.081 & 0.078 & 0.079 & 0.081 & 0.078 & 0.083 & 0.081 & 0.080 \\
\SwinUNETR\ \TTE\ & \textbf{0.069} & \textbf{0.067} & \textbf{0.066} & \textbf{0.069} & \textbf{0.067} & \textbf{0.073} & \textbf{0.079} & \textbf{0.069} \\
\midrule
\DenseNet\ \base\ & 0.219 & 0.803 & 0.702 & 0.779 & 0.217 & 0.533 & 0.335 & 0.822 \\
\DenseNet\ \MT\  & 0.071 & 0.067 & 0.068 & 0.068 & 0.065 & 0.072 & 0.083 & 0.068 \\
\DenseNet\ \TTE\  & \textbf{0.028} & \textbf{0.021} & \textbf{0.022} & \textbf{0.014} & \textbf{0.014} & \textbf{0.029} & \textbf{0.023} & \textbf{0.014} \\
\midrule
\ResNet\ \base\ & 0.349 & 0.078 & 0.493 & 0.174 & 0.165 & 0.166 & 0.140 & 0.109 \\
\ResNet\ \MT\  & 0.077 & \textbf{0.074} & 0.078 & 0.075 & 0.074 & 0.077 & 0.078 & 0.077 \\
\ResNet\ \TTE\  & \textbf{0.075} & 0.077 & \textbf{0.074} & \textbf{0.068} & \textbf{0.067} & \textbf{0.077} & \textbf{0.074} & \textbf{0.071} \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Time-to-event} performance on INSPECT dataset for proposed method and baselines, measured by integrated Brier score (the lower the better).}
\label{tab:performance_metrics_time_dependent}
\end{table*}



==> tables/OLD/time_dependent_c_stats.tex <==
\begin{table*}[h!]
\centering
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{l c c c c c c c c}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{8}{c}{\textbf{Time-dependent c-statistics} \uparrow } \\
\cmidrule(lr){2-9}
 & \textbf{Mortality} & \textbf{Readmission} & \textbf{Pulmonary Hypertension} & \textbf{Atelectasis} & \textbf{Cardiomegaly} & \textbf{Consolidation} & \textbf{Edema} & \textbf{Pleural Effusion} \\
\midrule
\SwinUNETR\ \base\ & 0.644 & 0.632 & 0.636 & 0.584 & 0.616 & 0.561 & 0.637 & 0.611 \\
\SwinUNETR\ \MT\  & 0.642 & 0.627 & 0.627 & 0.619 & 0.625 & 0.631 & 0.640 & 0.632 \\
\SwinUNETR\ \TTE\ & \textbf{0.665} & \textbf{0.652} & \textbf{0.650} & \textbf{0.662} & \textbf{0.660} & \textbf{0.663} & \textbf{0.667} & \textbf{0.671} \\
\midrule
\DenseNet\ \base\ & 0.499 & 0.470 & 0.532 & 0.492 & 0.498 & 0.508 & 0.489 & 0.531 \\
\DenseNet\ \MT\  & 0.598 & 0.587 & 0.595 & 0.594 & 0.596 & 0.586 & 0.598 & 0.603 \\
\DenseNet\ \TTE\  & \textbf{0.677} & \textbf{0.657} & \textbf{0.658} & \textbf{0.651} & \textbf{0.648} & \textbf{0.651} & \textbf{0.658} & \textbf{0.657} \\
\midrule
\ResNet\ \base\ & 0.461 & 0.587 & 0.517 & 0.580 & 0.435 & 0.573 & 0.498 & 0.531 \\
\ResNet\ \MT\  & 0.632 & 0.600 & 0.621 & 0.615 & 0.604 & 0.620 & 0.618 & 0.606 \\
\ResNet\ \TTE\  & \textbf{0.652} & \textbf{0.636} & \textbf{0.621} & \textbf{0.638} & \textbf{0.631} & \textbf{0.635} & \textbf{0.640} & \textbf{0.641} \\
\bottomrule
\end{tabular}}
\caption{\textbf{Time-to-event} performance on INSPECT dataset for proposed method and baselines, measured by time-dependent c-statistics (the higher the better).}
\label{tab:performance_metrics_time_dependent}
\end{table*}

==> tables/auroc_inspect.tex <==
% \begin{table*}[!h]
% \centering
% \begin{tabular}{l c c c c c c c c}
% \toprule
% \multirow{2}{*}{Model} & PE & \multicolumn{3}{c}{Mortality} & \multicolumn{3}{c}{Readmission} & PH \\
% \cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-9}
% & 0M & 1M & 6M & 12M & 1M & 6M & 12M & 12M \\
% \midrule
% \SwinUNETR\ \base\ & 0.554 & 0.697 & 0.653 & 0.682 & 0.531 & 0.545 & 0.519 & 0.594 \\
% \SwinUNETR\ \MT\  & 0.609 & 0.754 & 0.705 & 0.698 & \underline{0.601} & 0.616 & 0.559 & 0.588 \\
% \SwinUNETR\ \SV\  & 0.580 & 0.657 & 0.703 & 0.701 & 0.588 & 0.594 & \underline{0.604} & 0.635 \\
% \SwinUNETR\  \TTE\ & \textbf{0.617} & \textbf{0.871} & \textbf{0.847} & \textbf{0.806} & \textbf{0.607} & \textbf{0.647} & \textbf{0.606} & \textbf{0.729} \\
% \midrule
% \DenseNet\ \base\ & 0.482 & 0.571 & 0.501 & 0.493 & 0.453 & 0.463 & 0.471 & 0.501 \\
% \DenseNet\ \MT\  & 0.514 & 0.675 & 0.661 & 0.657 & \underline{0.530} & 0.520 & 0.504 & 0.456 \\
% \DenseNet\ \SV\  & 0.490 & 0.625 & 0.526 & 0.517 & 0.540 & 0.525 & 0.576 & 0.522 \\
% \DenseNet\ \TTE\  & \textbf{0.614} & \textbf{0.806} & \textbf{0.772} & \textbf{0.753} & \textbf{0.571} & \textbf{0.575} & \textbf{0.576} & \textbf{0.646} \\
% \midrule
% \ResNet\ \base\ & 0.456 & 0.628 & 0.590 & 0.603 & 0.542 & 0.565 & 0.552 & 0.464 \\
% \ResNet\ \MT\  & 0.547 & 0.782 & 0.715 & 0.705 & \underline{0.565} & 0.546 & 0.537 & 0.608 \\
% \ResNet\ \SV\  & \textbf{0.606} & 0.804 & 0.768 & 0.754 & 0.540 & 0.559 & 0.559 & 0.627 \\
% \ResNet\ \TTE\  & \underline{0.605} & \textbf{0.813} & \textbf{0.775} & \textbf{0.761} & \textbf{0.574} & \textbf{0.573} & \textbf{0.570} & \textbf{0.661} \\
% \bottomrule
% \end{tabular}
% \caption{\fra{PE is here so diagnostic as well}Prognostic binary classification performance for INSPECT tasks (1, 6, 12 month time horizon bins) reported as the mean AUROC of a test set bootstrap (n=1000). \textbf{Bold} indicates the best performer. \underline{Underlined} indicates no statistically significant difference versus the $*_{\tt{base/TTE}}$ models.}
% \label{tbl:inspect_auroc}
% \end{table*}




\begin{table*}[!h]
\centering
\begin{tabular}{l c c c c c c c}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c}{Mortality} & \multicolumn{3}{c}{Readmission} & PH \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8}
& 1M & 6M & 12M & 1M & 6M & 12M & 12M \\
\midrule
\SwinUNETR\ \base\ & 0.697 & 0.653 & 0.682 & 0.531 & 0.545 & 0.519 & 0.594 \\
\SwinUNETR\ \MT\  & 0.754 & 0.705 & 0.698 & \underline{0.601} & 0.616 & 0.559 & 0.588 \\
\SwinUNETR\ \SV\  & 0.657 & 0.703 & 0.701 & 0.588 & 0.594 & \underline{0.604} & 0.635 \\
\SwinUNETR\  \TTE\ & \textbf{0.871} & \textbf{0.847} & \textbf{0.806} & \textbf{0.607} & \textbf{0.647} & \textbf{0.606} & \textbf{0.729} \\
\midrule
\DenseNet\ \base\ & 0.571 & 0.501 & 0.493 & 0.453 & 0.463 & 0.471 & 0.501 \\
DenseNet ETHAN \base\ & 0.616 & 0.567 & 0.576 & 0.512 & 0.531 & 0.524 & 0.506 \\
\DenseNet\ \MT\  & 0.675 & 0.661 & 0.657 & \underline{0.530} & 0.520 & 0.504 & 0.456 \\
\DenseNet\ \SV\  & 0.625 & 0.526 & 0.517 & 0.540 & 0.525 & 0.576 & 0.522 \\
\DenseNet\ \TTE\  & \textbf{0.806} & \textbf{0.772} & \textbf{0.753} & \textbf{0.571} & \textbf{0.575} & \textbf{0.576} & \textbf{0.646} \\
\midrule
\ResNet\ \base\ & 0.628 & 0.590 & 0.603 & 0.542 & 0.565 & 0.552 & 0.464 \\
\ResNet\ \MT\  & 0.782 & 0.715 & 0.705 & \underline{0.565} & 0.546 & 0.537 & 0.608 \\
\ResNet\ \SV\  & 0.804 & 0.768 & 0.754 & 0.540 & 0.559 & 0.559 & 0.627 \\
\ResNet\ \TTE\  & \textbf{0.813} & \textbf{0.775} & \textbf{0.761} & \textbf{0.574} & \textbf{0.573} & \textbf{0.570} & \textbf{0.661} \\
\bottomrule
\end{tabular}
\caption{Prognostic binary classification performance for INSPECT tasks (1, 6, 12 month time horizon bins) reported as the mean AUROC of a test set bootstrap (n=1000). \textbf{Bold} indicates the best performer. \underline{Underlined} indicates no statistically significant difference versus the $*_{\tt{base/TTE}}$ models.}
\label{tbl:inspect_auroc}
\end{table*}


==> tables/auroc_rsna.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{l c c c c c c c c}
\toprule
\multirow{2}{*}{Model} & \multicolumn{6}{c}{PE} & \multicolumn{2}{c}{RV/LV Ratio} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-9}
& Left & Cent. & Right & Chronic & Acute & Indet. & $<$1 & $\geq$1 \\
\midrule
\SwinUNETR\ \base\ & \underline{0.526}& \underline{0.638}& \underline{0.566}& \underline{0.436} & \underline{0.568} & 0.413 & \underline{0.531} & 0.545 \\
\SwinUNETR\ \MT\ & \underline{0.521} & \underline{0.630} & 0.541 & 0.430 & \textbf{0.576} & \underline{0.666} & \underline{0.531} & 0.517 \\
\SwinUNETR\ \SV\ & \underline{\textbf{0.562}} & \underline{{0.648}} & \underline{0.549} & \underline{0.553} & \underline{0.542} & 0.634 & \underline{0.512} & 0.520 \\
\SwinUNETR\ \TTE\ & 0.539 & \textbf{0.649} & \textbf{0.583} & \textbf{0.554} & {0.535} & \textbf{0.536} & \textbf{0.673} & \textbf{0.598} \\
\midrule
\DenseNet\ \base\ & 0.508 & 0.581 & 0.500 & 0.493 & 0.405 & 0.419 & 0.484 & 0.493 \\
\DenseNet\ \MT\ & \underline{0.552} & 0.618 & \underline{0.596} & 0.528 & 0.478 & 0.492 & \underline{0.543}& 0.574 \\
\DenseNet\ \SV\ & \underline{0.558} & 0.553 & 0.551 & \textbf{0.572} & 0.452 & \underline{\textbf{0.666}} & \underline{0.520} & 0.549 \\
\DenseNet\ \TTE\ & \textbf{0.565} & \textbf{0.681} & \textbf{0.599} & 0.504 & \textbf{0.535} & \textbf{0.545} & \textbf{0.658} & \textbf{0.631} \\
\midrule
\ResNet\ \base\ & 0.585 & \underline{0.648}& \underline{\textbf{0.589}} & \underline{0.475} & \underline{0.483} & \underline{0.665} & \underline{0.530} & 0.589 \\
\ResNet\ \MT\ & \textbf{0.589} & 0.559 & 0.512 & \underline{0.425} & \underline{0.479} & 0.696 & \underline{0.511} & 0.623 \\
\ResNet\ \SV\ & 0.586 & {0.661} & \underline{0.584} & \underline{0.491} & \underline{0.479} & \underline{0.696} & \textbf{0.583} & \underline{0.590} \\
\ResNet\ \TTE\ & 0.527 & \textbf{0.663} & 0.580 & \textbf{0.620} & \textbf{0.505} & \textbf{0.700} & 0.546 & \textbf{0.644} \\
\bottomrule
\end{tabular}
\caption{Diagnostic binary classification performance for RSPECT, reported as the mean AUROC of a test set bootstrap (n=1000). \textbf{Bold} indicates the best performer. \underline{Underlined} indicates no statistically significant difference versus the $*_{\tt{base/TTE}}$ models.}
\label{tbl:rspect_auroc}
\end{table*}

